Investigation into Target Speaking Rate Adaptation for Voice Conversion

Disentangling speaker and content attributes of a speech signal into separate latent representations followed by decoding the content with an exchanged speaker representation is a popular approach for voice conversion, which can be trained with non-parallel and unlabeled speech data. However, previous approaches perform disentanglement only implicitly via some sort of information bottleneck or normalization, where it is usually hard to find a good trade-off between voice conversion and content reconstruction. Further, previous works usually do not consider an adaptation of the speaking rate to the target speaker or they put some major restrictions to the data or use case. Therefore, the contribution of this work is two-fold. First, we employ an explicit and fully unsupervised disentanglement approach, which has previously only been used for representation learning, and show that it allows to obtain both superior voice conversion and content reconstruction. Second, we investigate simple and generic approaches to linearly adapt the length of a speech signal, and hence the speaking rate, to a target speaker and show that the proposed adaptation allows to increase the speaking rate similarity with respect to the target speaker.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> figures/histogram_duration_diff.tex <==
% This file was created by tikzplotlib v0.9.5.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0,1}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1,0.5)}, anchor=south west, draw=white!80!black},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xmin=-0.75, xmax=15.75,
xtick style={color=black},
xtick={2.5,7.5,12.5},
xticklabels={S2F,F2S,N2N},
y grid style={white!69.0196078431373!black},
ylabel={Relative duration diff. to target},
ymajorgrids,
ymin=-0.404663342396805, ymax=0.699128844067751,
ytick style={color=black}
]
\path [draw=black, line width=0.52pt, dash pattern=on 4.81pt off 2.08pt]
(axis cs:0,0.05)
--(axis cs:15,0.05);

\path [draw=black, line width=0.52pt, dash pattern=on 4.81pt off 2.08pt]
(axis cs:0,-0.05)
--(axis cs:15,-0.05);

\addplot [blue, forget plot]
table {%
0.7 -0.0186187434546603
1.3 -0.0186187434546603
1.3 0.114851702746171
0.7 0.114851702746171
0.7 -0.0186187434546603
};
\addplot [blue, forget plot]
table {%
1 -0.0186187434546603
1 -0.202716669127418
};
\addplot [blue, forget plot]
table {%
1 0.114851702746171
1 0.207593199664557
};
\addplot [blue, forget plot]
table {%
0.85 -0.202716669127418
1.15 -0.202716669127418
};
\addplot [blue, forget plot]
table {%
0.85 0.207593199664557
1.15 0.207593199664557
};
\addplot [red, forget plot]
table {%
1.7 -0.0350485318604557
2.3 -0.0350485318604557
2.3 0.273461919646261
1.7 0.273461919646261
1.7 -0.0350485318604557
};
\addplot [red, forget plot]
table {%
2 -0.0350485318604557
2 -0.0766175740526229
};
\addplot [red, forget plot]
table {%
2 0.273461919646261
2 0.542810904768089
};
\addplot [red, forget plot]
table {%
1.85 -0.0766175740526229
2.15 -0.0766175740526229
};
\addplot [red, forget plot]
table {%
1.85 0.542810904768089
2.15 0.542810904768089
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
2.7 -0.0769029043466859
3.3 -0.0769029043466859
3.3 0.0579454079976923
2.7 0.0579454079976923
2.7 -0.0769029043466859
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
3 -0.0769029043466859
3 -0.188889878944488
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
3 0.0579454079976923
3 0.161557962664208
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
2.85 -0.188889878944488
3.15 -0.188889878944488
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
2.85 0.161557962664208
3.15 0.161557962664208
};
\addplot [color0, forget plot]
table {%
3.7 0.179944591841222
4.3 0.179944591841222
4.3 0.484660799376642
3.7 0.484660799376642
3.7 0.179944591841222
};
\addplot [color0, forget plot]
table {%
4 0.179944591841222
4 0.0904670375132066
};
\addplot [color0, forget plot]
table {%
4 0.484660799376642
4 0.648956471955726
};
\addplot [color0, forget plot]
table {%
3.85 0.0904670375132066
4.15 0.0904670375132066
};
\addplot [color0, forget plot]
table {%
3.85 0.648956471955726
4.15 0.648956471955726
};
\addplot [blue, forget plot]
table {%
5.7 -0.133945184387262
6.3 -0.133945184387262
6.3 0.0130916872287721
5.7 0.0130916872287721
5.7 -0.133945184387262
};
\addplot [blue, forget plot]
table {%
6 -0.133945184387262
6 -0.242760173278303
};
\addplot [blue, forget plot]
table {%
6 0.0130916872287721
6 0.140750129630697
};
\addplot [blue, forget plot]
table {%
5.85 -0.242760173278303
6.15 -0.242760173278303
};
\addplot [blue, forget plot]
table {%
5.85 0.140750129630697
6.15 0.140750129630697
};
\addplot [red, forget plot]
table {%
6.7 -0.26321169895623
7.3 -0.26321169895623
7.3 -0.0693486375542468
6.7 -0.0693486375542468
6.7 -0.26321169895623
};
\addplot [red, forget plot]
table {%
7 -0.26321169895623
7 -0.315178580511276
};
\addplot [red, forget plot]
table {%
7 -0.0693486375542468
7 0.0940830788730771
};
\addplot [red, forget plot]
table {%
6.85 -0.315178580511276
7.15 -0.315178580511276
};
\addplot [red, forget plot]
table {%
6.85 0.0940830788730771
7.15 0.0940830788730771
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
7.7 -0.0904860377307211
8.3 -0.0904860377307211
8.3 0.0283212439273293
7.7 0.0283212439273293
7.7 -0.0904860377307211
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
8 -0.0904860377307211
8 -0.144113129601186
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
8 0.0283212439273293
8 0.234177215189873
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
7.85 -0.144113129601186
8.15 -0.144113129601186
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
7.85 0.234177215189873
8.15 0.234177215189873
};
\addplot [color0, forget plot]
table {%
8.7 -0.315504104656013
9.3 -0.315504104656013
9.3 -0.158688602522158
8.7 -0.158688602522158
8.7 -0.315504104656013
};
\addplot [color0, forget plot]
table {%
9 -0.315504104656013
9 -0.35449097028478
};
\addplot [color0, forget plot]
table {%
9 -0.158688602522158
9 -0.0830132080380783
};
\addplot [color0, forget plot]
table {%
8.85 -0.35449097028478
9.15 -0.35449097028478
};
\addplot [color0, forget plot]
table {%
8.85 -0.0830132080380783
9.15 -0.0830132080380783
};
\addplot [blue, forget plot]
table {%
10.7 -0.0768460829695973
11.3 -0.0768460829695973
11.3 0.00853871349422319
10.7 0.00853871349422319
10.7 -0.0768460829695973
};
\addplot [blue, forget plot]
table {%
11 -0.0768460829695973
11 -0.128642368593648
};
\addplot [blue, forget plot]
table {%
11 0.00853871349422319
11 0.0484276140437526
};
\addplot [blue, forget plot]
table {%
10.85 -0.128642368593648
11.15 -0.128642368593648
};
\addplot [blue, forget plot]
table {%
10.85 0.0484276140437526
11.15 0.0484276140437526
};
\addplot [red, forget plot]
table {%
11.7 -0.0630475431433924
12.3 -0.0630475431433924
12.3 0.129954089759205
11.7 0.129954089759205
11.7 -0.0630475431433924
};
\addplot [red, forget plot]
table {%
12 -0.0630475431433924
12 -0.103690685413005
};
\addplot [red, forget plot]
table {%
12 0.129954089759205
12 0.244624594449601
};
\addplot [red, forget plot]
table {%
11.85 -0.103690685413005
12.15 -0.103690685413005
};
\addplot [red, forget plot]
table {%
11.85 0.244624594449601
12.15 0.244624594449601
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
12.7 -0.0685092059792258
13.3 -0.0685092059792258
13.3 0.0386391580904065
12.7 0.0386391580904065
12.7 -0.0685092059792258
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
13 -0.0685092059792258
13 -0.106155720041226
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
13 0.0386391580904065
13 0.100542436964056
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
12.85 -0.106155720041226
13.15 -0.106155720041226
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
12.85 0.100542436964056
13.15 0.100542436964056
};
\addplot [color0, forget plot]
table {%
13.7 -0.0454549855260483
14.3 -0.0454549855260483
14.3 0.034041365093984
13.7 0.034041365093984
13.7 -0.0454549855260483
};
\addplot [color0, forget plot]
table {%
14 -0.0454549855260483
14 -0.0880348381131344
};
\addplot [color0, forget plot]
table {%
14 0.034041365093984
14 0.0671294191345114
};
\addplot [color0, forget plot]
table {%
13.85 -0.0880348381131344
14.15 -0.0880348381131344
};
\addplot [color0, forget plot]
table {%
13.85 0.0671294191345114
14.15 0.0671294191345114
};
\addplot [blue, forget plot]
table {%
0.7 0.0696309904303081
1.3 0.0696309904303081
};
\addplot [red, forget plot]
table {%
1.7 0.183833116036506
2.3 0.183833116036506
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
2.7 -0.0132024080081886
3.3 -0.0132024080081886
};
\addplot [color0, forget plot]
table {%
3.7 0.327155374463635
4.3 0.327155374463635
};
\addplot [blue, forget plot]
table {%
5.7 -0.0881254895577958
6.3 -0.0881254895577958
};
\addplot [red, forget plot]
table {%
6.7 -0.134972987036839
7.3 -0.134972987036839
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
7.7 -0.0441797300184125
8.3 -0.0441797300184125
};
\addplot [color0, forget plot]
table {%
8.7 -0.25185672210556
9.3 -0.25185672210556
};
\addplot [blue, forget plot]
table {%
10.7 -0.0554657320721471
11.3 -0.0554657320721471
};
\addplot [red, forget plot]
table {%
11.7 0.0804635537182081
12.3 0.0804635537182081
};
\addplot [green!50.1960784313725!black, forget plot]
table {%
12.7 -0.0418398336981045
13.3 -0.0418398336981045
};
\addplot [color0, forget plot]
table {%
13.7 -0.0346566138849249
14.3 -0.0346566138849249
};
\end{axis}

\end{tikzpicture}

